Universality, criticality and complexity of information propagation in social media

Information avalanches in social media are typically studied in a similar fashion as avalanches of neuronal activity in the brain. Whereas a large body of literature reveals substantial agreement about the existence of a unique process characterizing neuronal activity across organisms, the dynamics of information in online social media is far less understood. Statistical laws of information avalanches are found in previous studies to be not robust across systems, and radically different processes are used to represent plausible driving mechanisms for information propagation. Here, we analyze almost 1 billion time-stamped events collected from a multitude of online platforms -- including Telegram, Twitter and Weibo -- over observation windows longer than 10 years to show that the propagation of information in social media is a universal and critical process. Universality arises from the observation of identical macroscopic patterns across platforms, irrespective of the details of the specific system at hand. Critical behavior is deduced from the power-law distributions, and corresponding hyperscaling relations, characterizing size and duration of avalanches of information. Neuronal activity may be modeled as a simple contagion process, where only a single exposure to activity may be sufficient for its diffusion. On the contrary, statistical testing on our data indicates that a mixture of simple and complex contagion, where involvement of an individual requires exposure from multiple acquaintances, characterizes the propagation of information in social media. We show that the complexity of the process is correlated with the semantic content of the information that is propagated. Conversational topics about music, movies and TV shows tend to propagate as simple contagion processes, whereas controversial discussions on political/societal themes obey the rules of complex contagion.

==> biblio.tex <==
@MISC{osome,
title = {{OS}o{M}e, {O}bservatory on {S}ocial {M}edia},
author={Indiana University},
year={2020},
howpublished={\url{https://osome.iu.edu}}
}

@MISC{twitterdeca,
title = {Twitter, {D}ecahose stream},
howpublished={\url{https://developer.twitter.com/en/docs/twitter-api/v1/tweets/sample-realtime/overview/decahose}}
}

@article{radicchi2020classes,
  title={Classes of critical avalanche dynamics in complex networks},
  author={Radicchi, Filippo and Castellano, Claudio and Flammini, Alessandro and Mu{\~n}oz, Miguel A and Notarmuzi, Daniele},
  journal={Physical Review Research},
  volume={2},
  number={3},
  pages={033171},
  year={2020},
  publisher={APS}
}

@article{dalla2019modeling,
  title={Modeling neuronal avalanches and long-range temporal correlations at the emergence of collective oscillations: Continuously varying exponents mimic M/EEG results},
  author={Dalla Porta, Leonardo and Copelli, Mauro},
  journal={PLoS computational biology},
  volume={15},
  number={4},
  pages={e1006924},
  year={2019},
  publisher={Public Library of Science}
}

@article{beggs2003neuronal,
  title={Neuronal avalanches in neocortical circuits},
  author={Beggs, John M and Plenz, Dietmar},
  journal={Journal of neuroscience},
  volume={23},
  number={35},
  pages={11167--11177},
  year={2003},
  publisher={Soc Neuroscience}
}

@article{bak2002unified,
  title={Unified scaling law for earthquakes},
  author={Bak, Per and Christensen, Kim and Danon, Leon and Scanlon, Tim},
  journal={Physical Review Letters},
  volume={88},
  number={17},
  pages={178501},
  year={2002},
  publisher={APS}
}

@article{dodds2005generalized,
  title={A generalized model of social and biological contagion},
  author={Dodds, Peter Sheridan and Watts, Duncan J},
  journal={Journal of theoretical biology},
  volume={232},
  number={4},
  pages={587--604},
  year={2005},
  publisher={Elsevier}
}

@article{munoz1999avalanche,
  title={Avalanche and spreading exponents in systems with absorbing states},
  author={Munoz, Miguel A and Dickman, Ronald and Vespignani, Alessandro and Zapperi, Stefano},
  journal={Physical Review E},
  volume={59},
  number={5},
  pages={6175},
  year={1999},
  publisher={APS}
}

@article{ahmad2010twitter,
  title={Is Twitter a useful tool for journalists?},
  author={Ahmad, Ali Nobil},
  journal={Journal of media practice},
  volume={11},
  number={2},
  pages={145--155},
  year={2010},
  publisher={Taylor \& Francis}
}

@article{odor2004universality,
  title={Universality classes in nonequilibrium lattice systems},
  author={{\'O}dor, G{\'e}za},
  journal={Reviews of Modern Physics},
  volume={76},
  number={3},
  pages={663},
  year={2004},
  publisher={APS}
}

@article{centola2007complex,
  title={Complex contagions and the weakness of long ties},
  author={Centola, Damon and Macy, Michael},
  journal={American journal of Sociology},
  volume={113},
  number={3},
  pages={702--734},
  year={2007},
  publisher={The University of Chicago Press}
}

@inproceedings{romero2011differences,
  title={Differences in the mechanics of information diffusion across topics: idioms, political hashtags, and complex contagion on twitter},
  author={Romero, Daniel M and Meeder, Brendan and Kleinberg, Jon},
  booktitle={Proceedings of the 20th international conference on World wide web},
  pages={695--704},
  year={2011}
}

@inproceedings{weng2014predicting,
  title={Predicting successful memes using network and community structure},
  author={Weng, Lilian and Menczer, Filippo and Ahn, Yong-Yeol},
  booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
  volume={8},
  number={1},
  year={2014}
}

@article{vasconcelos2019consensus,
  title={Consensus and polarization in competing complex contagion processes},
  author={Vasconcelos, V{\'\i}tor V and Levin, Simon A and Pinheiro, Fl{\'a}vio L},
  journal={Journal of the Royal Society Interface},
  volume={16},
  number={155},
  pages={20190196},
  year={2019},
  publisher={The Royal Society}
}

@inproceedings{kobayashi2016tideh,
  title={Tideh: Time-dependent hawkes process for predicting retweet dynamics},
  author={Kobayashi, Ryota and Lambiotte, Renaud},
  booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
  volume={10},
  number={1},
  year={2016}
}

@inproceedings{zhao2015seismic,
  title={Seismic: A self-exciting point process model for predicting tweet popularity},
  author={Zhao, Qingyuan and Erdogdu, Murat A and He, Hera Y and Rajaraman, Anand and Leskovec, Jure},
  booktitle={Proceedings of the 21th ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={1513--1522},
  year={2015}
}

@inproceedings{matsubara2012rise,
  title={Rise and fall patterns of information diffusion: model and implications},
  author={Matsubara, Yasuko and Sakurai, Yasushi and Prakash, B Aditya and Li, Lei and Faloutsos, Christos},
  booktitle={Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={6--14},
  year={2012}
}

@inproceedings{rizoiu2017expecting,
  title={Expecting to be hip: Hawkes intensity processes for social media popularity},
  author={Rizoiu, Marian-Andrei and Xie, Lexing and Sanner, Scott and Cebrian, Manuel and Yu, Honglin and Van Hentenryck, Pascal},
  booktitle={Proceedings of the 26th International Conference on World Wide Web},
  pages={735--744},
  year={2017}
}

@article{haimovich2020scalable,
  title={Scalable Prediction of Information Cascades over Arbitrary Time Horizons},
  author={Haimovich, Daniel and Karamshuk, Dima and Leeper, Thomas J and Riabenko, Evgeniy and Vojnovic, Milan},
  journal={arXiv preprint arXiv:2009.02092},
  year={2020}
}

@article{notarmuzi2021percolation,
  title={Percolation theory of self-exciting temporal processes},
  author={Notarmuzi, Daniele and Castellano, Claudio and Flammini, Alessandro and Mazzilli, Dario and Radicchi, Filippo},
  journal={Physical Review E},
  volume={103},
  number={2},
  pages={L020302},
  year={2021},
  publisher={APS}
}

@misc{Howell2013digital,
  title={Digital wildfires in a hyperconnected world},
  author={Lee Howell et al. In Global Risks. World Economic Forum},
  howpublished={http://reports.weforum.org/global-risks-2013/risk-case-1/digital-wildfires-in-a-hyperconnected-world/},
  year={2013}
}


@inproceedings{kwak2010twitter,
  title={What is Twitter, a social network or a news media?},
  author={Kwak, Haewoon and Lee, Changhyun and Park, Hosung and Moon, Sue},
  booktitle={Proceedings of the 19th international conference on World wide web},
  pages={591--600},
  year={2010}
}


@article{pierri2021impact,
  title={The impact of online misinformation on US COVID-19 vaccinations},
  author={Pierri, Francesco and Perry, Brea and DeVerna, Matthew R and Yang, Kai-Cheng and Flammini, Alessandro and Menczer, Filippo and Bryden, John},
  journal={arXiv preprint arXiv:2104.10635},
  year={2021}
}

@article{yang2020prevalence,
  title={Prevalence of low-credibility information on twitter during the covid-19 outbreak},
  author={Yang, Kai-Cheng and Torres-Lugo, Christopher and Menczer, Filippo},
  journal={arXiv preprint arXiv:2004.14484},
  year={2020}
}

@article{yang2021covid,
  title={The COVID-19 Infodemic: Twitter versus Facebook},
  author={Yang, Kai-Cheng and Pierri, Francesco and Hui, Pik-Mai and Axelrod, David and Torres-Lugo, Christopher and Bryden, John and Menczer, Filippo},
  journal={Big Data \& Society},
  volume={8},
  number={1},
  pages={20539517211013861},
  year={2021},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{bessi2016social,
  title={Social bots distort the 2016 US Presidential election online discussion},
  author={Bessi, Alessandro and Ferrara, Emilio},
  journal={First Monday},
  volume={21},
  number={11-7},
  year={2016}
}

@article{metaxas2012social,
  title={Social media and the elections},
  author={Metaxas, Panagiotis T and Mustafaraj, Eni},
  journal={Science},
  volume={338},
  number={6106},
  pages={472--473},
  year={2012},
  publisher={American Association for the Advancement of Science}
}


@article{barabasi2005origin,
  title={The origin of bursts and heavy tails in human dynamics},
  author={Barabasi, Albert-Laszlo},
  journal={Nature},
  volume={435},
  number={7039},
  pages={207--211},
  year={2005},
  publisher={Nature Publishing Group}
}

@inproceedings{lerman2010information,
  title={Information contagion: An empirical study of the spread of news on digg and twitter social networks},
  author={Lerman, Kristina and Ghosh, Rumi},
  booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
  volume={4},
  number={1},
  year={2010}
}

@article{onnela2010spontaneous,
  title={Spontaneous emergence of social influence in online systems},
  author={Onnela, Jukka-Pekka and Reed-Tsochas, Felix},
  journal={Proceedings of the National Academy of Sciences},
  volume={107},
  number={43},
  pages={18375--18380},
  year={2010},
  publisher={National Acad Sciences}
}

@article{munoz2018colloquium,
  title={Colloquium: Criticality and dynamical scaling in living systems},
  author={Munoz, Miguel A},
  journal={Reviews of Modern Physics},
  volume={90},
  number={3},
  pages={031001},
  year={2018},
  publisher={APS}
}


@article{colaiori2008exactly,
  title={Exactly solvable model of avalanches dynamics for Barkhausen crackling noise},
  author={Colaiori, Francesca},
  journal={Advances in Physics},
  volume={57},
  number={4},
  pages={287--359},
  year={2008},
  publisher={Taylor \& Francis}
}

@article{gleeson2014competition,
  title={Competition-induced criticality in a model of meme popularity},
  author={Gleeson, James P and Ward, Jonathan A and O’sullivan, Kevin P and Lee, William T},
  journal={Physical review letters},
  volume={112},
  number={4},
  pages={048701},
  year={2014},
  publisher={APS}
}

@article{gleeson2016effects,
  title={Effects of network structure, competition and memory time on social spreading phenomena},
  author={Gleeson, James P and O’Sullivan, Kevin P and Ba{\~n}os, Raquel A and Moreno, Yamir},
  journal={Physical Review X},
  volume={6},
  number={2},
  pages={021019},
  year={2016},
  publisher={APS}
}


@article{o2020quantifying,
	Author = {O'Brien, Joseph D and Aleta, Alberto and Moreno, Yamir and Gleeson, James P},
	Date-Added = {2020-02-20 14:41:40 +0000},
	Date-Modified = {2020-02-20 14:41:40 +0000},
	Journal = {arXiv preprint arXiv:2001.09490},
	Title = {Quantifying Uncertainty in a Predictive Model for Popularity Dynamics},
	Year = {2020}
}
	
	
@article{qiu2017limited,
  title={Limited individual attention and online virality of low-quality information},
  author={Qiu, Xiaoyan and Oliveira, Diego FM and Shirazi, Alireza Sahami and Flammini, Alessandro and Menczer, Filippo},
  journal={Nature Human Behaviour},
  volume={1},
  number={7},
  pages={1--7},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{sreenivasan2016information,
  title={Information cascades in feed-based networks of users with limited attention},
  author={Sreenivasan, Sameet and Chan, Kevin S and Swami, Ananthram and Korniss, Gyorgy and Szymanski, Boleslaw Karol},
  journal={IEEE Transactions on Network Science and Engineering},
  volume={4},
  number={2},
  pages={120--128},
  year={2016},
  publisher={IEEE}
}

@article{nishi2016reply,
  title={Reply trees in twitter: data analysis and branching process models},
  author={Nishi, Ryosuke and Takaguchi, Taro and Oka, Keigo and Maehara, Takanori and Toyoda, Masashi and Kawarabayashi, Ken-ichi and Masuda, Naoki},
  journal={Social Network Analysis and Mining},
  volume={6},
  number={1},
  pages={26},
  year={2016},
  publisher={Springer}
}

@article{crane2008robust,
  title={Robust dynamic classes revealed by measuring the response function of a social system},
  author={Crane, Riley and Sornette, Didier},
  journal={Proceedings of the National Academy of Sciences},
  volume={105},
  number={41},
  pages={15649--15653},
  year={2008},
  publisher={National Acad Sciences}
}

@article{watson1875probability,
  title={On the probability of the extinction of families},
  author={Watson, Henry William and Galton, Francis},
  journal={The Journal of the Anthropological Institute of Great Britain and Ireland},
  volume={4},
  pages={138--144},
  year={1875},
  publisher={JSTOR}
}

@book{harris1963theory,
  title={The theory of branching processes},
  author={Harris, Theodore Edward and others},
  volume={6},
  year={1963},
  publisher={Springer Berlin}
}

@book{liggett2012interacting,
  title={Interacting particle systems},
  author={Liggett, Thomas Milton},
  volume={276},
  year={2012},
  publisher={Springer Science \& Business Media}
}


@article{fontenele2019criticality,
  title={Criticality between cortical states},
  author={Fontenele, Antonio J and de Vasconcelos, Nivaldo AP and Feliciano, Tha{\'\i}s and Aguiar, Leandro AA and Soares-Cunha, Carina and Coimbra, B{\'a}rbara and Dalla Porta, Leonardo and Ribeiro, Sidarta and Rodrigues, Ana Jo{\~a}o and Sousa, Nuno and others},
  journal={Physical review letters},
  volume={122},
  number={20},
  pages={208101},
  year={2019},
  publisher={APS}
}

@article{ponce2018whole,
  title={Whole-brain neuronal activity displays crackling noise dynamics},
  author={Ponce-Alvarez, Adri{\'a}n and Jouary, Adrien and Privat, Martin and Deco, Gustavo and Sumbre, Germ{\'a}n},
  journal={Neuron},
  volume={100},
  number={6},
  pages={1446--1459},
  year={2018},
  publisher={Elsevier}
}

@article{di2017simple,
  title={Simple unified view of branching process statistics: Random walks in balanced logarithmic potentials},
  author={di Santo, Serena and Villegas, Pablo and Burioni, Raffaella and Mu{\~n}oz, Miguel A},
  journal={Physical Review E},
  volume={95},
  number={3},
  pages={032115},
  year={2017},
  publisher={APS}
}


@article{sethna2001crackling,
  title={Crackling noise},
  author={Sethna, James P and Dahmen, Karin A and Myers, Christopher R},
  journal={Nature},
  volume={410},
  number={6825},
  pages={242--250},
  year={2001},
  publisher={Nature Publishing Group}
}



@inproceedings{wegrzycki2017cascade,
  title={Why do cascade sizes follow a power-law?},
  author={Wegrzycki, Karol and Sankowski, Piotr and Pacuk, Andrzej and Wygocki, Piotr},
  booktitle={Proceedings of the 26th International Conference on World Wide Web},
  pages={569--576},
  year={2017}
}


@article{li2019infectivity,
  title={Infectivity enhances prediction of viral cascades in Twitter},
  author={Li, Weihua and Cranmer, Skyler J and Zheng, Zhiming and Mucha, Peter J},
  journal={PloS one},
  volume={14},
  number={4},
  pages={e0214453},
  year={2019},
  publisher={Public Library of Science San Francisco, CA USA}
}


@article{oliveiraa2019diffusion,
  title={Diffusion of Information in an Online Social Network with Limited Attention},
  author={Oliveiraa, Diego FM and Chana, Kevin S},
  journal={Information \& Security},
  volume={43},
  number={1},
  pages={362--374},
  year={2019},
  publisher={ProCon Ltd.}
}


@article{bild2015aggregate,
  title={Aggregate characterization of user behavior in Twitter and analysis of the retweet graph},
  author={Bild, David R and Liu, Yue and Dick, Robert P and Mao, Z Morley and Wallach, Dan S},
  journal={ACM Transactions on Internet Technology (TOIT)},
  volume={15},
  number={1},
  pages={1--24},
  year={2015},
  publisher={ACM New York, NY, USA}
}



@article{weng2012competition,
	title = {Competition among memes in a world with limited attention},
	volume = {2},
	copyright = {2012 The Author(s)},
	issn = {2045-2322},
	url = {https://www.nature.com/articles/srep00335},
	doi = {10.1038/srep00335},
	language = {en},
	number = {1},
	urldate = {2020-11-25},
	journal = {Scientific Reports},
	author = {Weng, L. and Flammini, A. and Vespignani, A. and Menczer, F.},
	month = mar,
	year = {2012},
	note = {Number: 1
Publisher: Nature Publishing Group},
	pages = {335},
}



@article{szabo2010predicting,
  title={Predicting the popularity of online content},
  author={Szabo, Gabor and Huberman, Bernardo A},
  journal={Communications of the ACM},
  volume={53},
  number={8},
  pages={80--88},
  year={2010},
  publisher={ACM New York, NY, USA}
}




@article{michard2005theory,
  title={Theory of collective opinion shifts: from smooth trends to abrupt swings},
  author={Michard, Quentin and Bouchaud, J-P},
  journal={The European Physical Journal B-Condensed Matter and Complex Systems},
  volume={47},
  number={1},
  pages={151--159},
  year={2005},
  publisher={Springer}
}


@article{weng2013virality,
  title={Virality prediction and community structure in social networks},
  author={Weng, Lilian and Menczer, Filippo and Ahn, Yong-Yeol},
  journal={Scientific reports},
  volume={3},
  number={1},
  pages={1--6},
  year={2013},
  publisher={Nature Publishing Group}
}


@article{pastor2015epidemic,
	Author = {Pastor-Satorras, Romualdo and Castellano, Claudio and Van Mieghem, Piet and Vespignani, Alessandro},
	Date-Added = {2018-11-15 23:09:43 +0000},
	Date-Modified = {2018-11-15 23:11:09 +0000},
	Journal = {Reviews of modern physics},
	Number = {3},
	Pages = {925},
	Title = {Epidemic process in compex networks},
	Volume = {87},
	Year = {2015}
}

@article{edrington2018tweeting,
  title={Tweeting a social movement: Black Lives Matter and its use of Twitter to share information, build community, and promote action},
  author={Edrington, Candice LaShara and Lee, Nicole},
  journal={The Journal of Public Interest Communications},
  volume={2},
  number={2},
  pages={289--289},
  year={2018}
}

@article{tillery2019kind,
  title={What kind of movement is Black lives matter? The view from Twitter},
  author={Tillery, Alvin B},
  journal={Journal of Race, Ethnicity and Politics},
  volume={4},
  number={2},
  pages={297--323},
  year={2019},
  publisher={Cambridge University Press}
}

@article{phillips2021dumb,
  title={‘Dumb Money’is on GameStop, and it’s Beating Wall Street at its Own Game},
  author={Phillips, Matt and Lorenz, Taylor},
  journal={The New York Times. https://www. nytimes. com/2021/01/27/business/gamestop-wall-street-bets. html},
  year={2021}
}

@article{granovetter1973strength,
  title={The strength of weak ties},
  author={Granovetter, Mark S},
  journal={American journal of sociology},
  volume={78},
  number={6},
  pages={1360--1380},
  year={1973},
  publisher={University of Chicago Press}
}

@article{clauset2009power,
  title={Power-law distributions in empirical data},
  author={Clauset, Aaron and Shalizi, Cosma Rohilla and Newman, Mark EJ},
  journal={SIAM review},
  volume={51},
  number={4},
  pages={661--703},
  year={2009},
  publisher={SIAM}
}


@article{aliapoulios2021early,
  title={An early look at the parler online social network},
  author={Aliapoulios, Max and Bevensee, Emmi and Blackburn, Jeremy and Bradlyn, Barry and De Cristofaro, Emiliano and Stringhini, Gianluca and Zannettou, Savvas},
  journal={arXiv preprint arXiv:2101.03820},
  year={2021}
}



@article{baumgartner2020pushshift,
  title={The Pushshift Telegram Dataset},
  author={Baumgartner, Jason and Zannettou, Savvas and Squire, Megan and Blackburn, Jeremy},
  journal={arXiv preprint arXiv:2001.08438},
  year={2020}
}




@article{basile_topical_2015,
	Author = {Basile, Valerio and Peroni, Silvio and Tamburini, Fabio and Vitali, Fabio},
	Date-Added = {2020-01-25 00:24:00 +0000},
	Date-Modified = {2020-01-25 00:24:00 +0000},
	Doi = {10.1177/0165551515585283},
	File = {55a4f9eb08ae81aec91327f8.pdf:files/253/55a4f9eb08ae81aec91327f8.pdf:application/pdf},
	Journal = {J. Information Science},
	Number = {4},
	Pages = {486--505},
	Title = {Topical tags vs non-topical tags: {Towards} a bipartite classification?},
	Url = {http://dx.doi.org/10.1177/0165551515585283},
	Volume = {41},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1177/0165551515585283}}


@article{fu2013assessing,
  title={Assessing censorship on microblogs in China: Discriminatory keyword analysis and the real-name registration policy},
  author={Fu, King-wa and Chan, Chung-hong and Chau, Michael},
  journal={IEEE Internet Computing},
  volume={17},
  number={3},
  pages={42--50},
  year={2013},
  publisher={IEEE}
}



@article{timme2016criticality,
  title={Criticality maximizes complexity in neural tissue},
  author={Timme, Nicholas M and Marshall, Najja J and Bennett, Nicholas and Ripp, Monica and Lautzenhiser, Edward and Beggs, John M},
  journal={Frontiers in physiology},
  volume={7},
  pages={425},
  year={2016},
  publisher={Frontiers}
}

@MISC{TLGdata,
author={Baumgartner, Jason and Zannettou, Savvas and Squire, Megan and Blackburn, Jeremy},
year={2020},
howpublished={\url{https://zenodo.org/record/3607497#.YRu-4tMza-s}}
}


@MISC{PARLdata,
author={Aliapoulios, Max and Bevensee, Emmi and Blackburn, Jeremy and Bradlyn, Barry and De Cristofaro, Emiliano and Stringhini, Gianluca and Zannettou, Savvas},
year={2021},
howpublished={\url{https://zenodo.org/record/4442460#.YRu_WtMza-s}}
}


@MISC{TWTdata,
author={Notarmuzi, Daniele and Castellano, Claudio and Flammini, Alessandro and Mazzilli, Dario and Radicchi, Filippo},
year={2021},
howpublished={\url{https://github.com/DaniMuzi/SocialMedia}}
}



@MISC{DELdata,
author={Basile, Valerio},
year={2015},
howpublished={\url{http://valeriobasile.github.io/delicious/}}
}




@MISC{SOdata,
title = {Link to StackOverflow data},
howpublished={\url{https://archive.org/download/stackexchange/stackoverflow.com-Posts.7z}}
}



@MISC{WEIdata,
title = {Weiboscope Open Data. (Dataset)},
author={Fu, King-wa},
year={2017},
publisher={The University of Hong Kong, Pokfulam, Hong Kong SA},
howpublished={\url{https://hub.hku.hk/cris/dataset/dataset107483}}
}


@article{karsai2012universal,
  title={Universal features of correlated bursty behaviour},
  author={Karsai, M{\'a}rton and Kaski, Kimmo and Barab{\'a}si, Albert-L{\'a}szl{\'o} and Kert{\'e}sz, J{\'a}nos},
  journal={Scientific reports},
  volume={2},
  number={1},
  pages={1--7},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{touboul2017power,
  title={Power-law statistics and universal scaling in the absence of criticality},
  author={Touboul, Jonathan and Destexhe, Alain},
  journal={Physical Review E},
  volume={95},
  number={1},
  pages={012413},
  year={2017},
  publisher={APS}
}


@article{destexhe2020comment,
  title={Comment on" Criticality Between Cortical States"},
  author={Destexhe, Alain and Touboul, Jonathan D},
  journal={arXiv preprint arXiv:2002.08813},
  year={2020}
}

@inproceedings{state2015diffusion,
  title={The diffusion of support in an online social movement: Evidence from the adoption of equal-sign profile pictures},
  author={State, Bogdan and Adamic, Lada},
  booktitle={Proceedings of the 18th ACM Conference on Computer Supported Cooperative Work \& Social Computing},
  pages={1741--1750},
  year={2015}
}



@MISC{RHDCdata,
title = {Dissociated cutlures of rat's hippocampal cells (Dataset)},
author={Timme, Nicholas M and Marshall, Najja J and Bennett, Nicholas and Ripp, Monica and Lautzenhiser, Edward and Beggs, John M},
year={2016},
howpublished={\url{https://crcns.org/data-sets/hc/hc-8}}
}

@article{ito2014large,
  title={Large-scale, high-resolution multielectrode-array recording depicts functional network differences of cortical and hippocampal cultures},
  author={Ito, Shinya and Yeh, Fang-Chin and Hiolski, Emma and Rydygier, Przemyslaw and Gunning, Deborah E and Hottowy, Pawel and Timme, Nicholas and Litke, Alan M and Beggs, John M},
  journal={PloS one},
  volume={9},
  number={8},
  pages={e105324},
  year={2014},
  publisher={Public Library of Science}
}

@article{litke2004does,
  title={What does the eye tell the brain?: Development of a system for the large-scale recording of retinal output activity},
  author={Litke, AM and Bezayiff, N and Chichilnisky, EJ and Cunningham, W and Dabrowski, W and Grillo, AA and Grivich, M and Grybos, P and Hottowy, P and Kachiguine, S and others},
  journal={IEEE Transactions on Nuclear Science},
  volume={51},
  number={4},
  pages={1434--1440},
  year={2004},
  publisher={IEEE}
}


@MISC{MSOSdata,
title = {Spontaneous spiking activity of hundreds of neurons in mouse somatosensory cortex slice cultures recorded using a dense 512 electrode array},
author={Shinya Ito and Fang-Chin Yeh and Nicholas M. Timme and Pawel Hottowy and Alan M. Litke and John M. Beggs},
year={2016},
publisher={CRCNS.org},
howpublished={\url{http://dx.doi.org/10.6080/K07D2S2F}}
}


 


@article{lawlor2018linear,
  title={Linear-nonlinear-time-warp-poisson models of neural activity},
  author={Lawlor, Patrick N and Perich, Matthew G and Miller, Lee E and Kording, Konrad P},
  journal={Journal of computational neuroscience},
  volume={45},
  number={3},
  pages={173--191},
  year={2018},
  publisher={Springer}
}



@MISC{MPCdata,
title = {Extracellular neural recordings from macaque primary and dorsal premotor motor cortex during a sequential reaching task.},
author={Matthew G. Perich and Patrick N. Lawlor and Konrad P. Kording and Lee E. Miller},
year={2018},
publisher={CRCNS.org},
howpublished={\url{http://dx.doi.org/10.6080/K0FT8J72}}
}


@MISC{JAPdata,
publisher={Earthquake Information Center,
Earthquake Research Institute, Yayoi 1-1-1, Bunkyo, Tokyo 113-0032, Japan},
howpublished={\url{http://wwweic.eri.u-tokyo.ac.jp/CATALOG/junec/monthly.html}}
}

@article{grunthal2013share,
  title={The SHARE European Earthquake Catalogue (SHEEC) for the time period 1900--2006 and its comparison to the European-Mediterranean Earthquake Catalogue (EMEC)},
  author={Gr{\"u}nthal, Gottfried and Wahlstr{\"o}m, Rutger and Stromeyer, Dietrich},
  journal={Journal of seismology},
  volume={17},
  number={4},
  pages={1339--1344},
  year={2013},
  publisher={Springer}
}

@MISC{EURdata,
title = {Data taken from SHEEC 1900-2006 (Grünthal et al., 2013)
.},
author={Gr{\"u}nthal, Gottfried and Wahlstr{\"o}m, Rutger and Stromeyer, Dietrich},
year={2013},
howpublished={\url{https://www.gfz-potsdam.de/sheec/}}
}


@MISC{CALdata,
title = {California Earthquakes (dataset)},
howpublished={\url{https://www.conservation.ca.gov/cgs/Documents/Melange/cgs2000_fnl.txt}}
}


@article{beggs2012being,
  title={Being critical of criticality in the brain},
  author={Beggs, John M and Timme, Nicholas},
  journal={Frontiers in physiology},
  volume={3},
  pages={163},
  year={2012},
  publisher={Frontiers}
}

@article{haldeman2005critical,
  title={Critical branching captures activity in living neural networks and maximizes the number of metastable states},
  author={Haldeman, Clayton and Beggs, John M},
  journal={Physical review letters},
  volume={94},
  number={5},
  pages={058101},
  year={2005},
  publisher={APS}
}

@article{friedman2012universal,
  title={Universal critical dynamics in high resolution neuronal avalanche data},
  author={Friedman, Nir and Ito, Shinya and Brinkman, Braden AW and Shimono, Masanori and DeVille, RE Lee and Dahmen, Karin A and Beggs, John M and Butler, Thomas C},
  journal={Physical review letters},
  volume={108},
  number={20},
  pages={208102},
  year={2012},
  publisher={APS}
}

@book{stauffer2018introduction,
  title={Introduction to percolation theory},
  author={Stauffer, Dietrich and Aharony, Ammon},
  year={2018},
  publisher={CRC press}
}

@article{guilbeault2018complex,
  title={Complex contagions: A decade in review},
  author={Guilbeault, Douglas and Becker, Joshua and Centola, Damon},
  journal={Complex spreading phenomena in social systems},
  pages={3--25},
  year={2018},
  publisher={Springer}
}




@inproceedings{cao2017deephawkes,
  title={Deephawkes: Bridging the gap between prediction and understanding of information cascades},
  author={Cao, Qi and Shen, Huawei and Cen, Keting and Ouyang, Wentao and Cheng, Xueqi},
  booktitle={Proceedings of the 2017 ACM on Conference on Information and Knowledge Management},
  pages={1149--1158},
  year={2017}
}


@article{zhou2021survey,
  title={A survey of information cascade analysis: Models, predictions, and recent advances},
  author={Zhou, Fan and Xu, Xovee and Trajcevski, Goce and Zhang, Kunpeng},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={2},
  pages={1--36},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{hodas2014simple,
  title={The simple rules of social contagion},
  author={Hodas, Nathan O and Lerman, Kristina},
  journal={Scientific reports},
  volume={4},
  number={1},
  pages={1--7},
  year={2014},
  publisher={Nature Publishing Group}
}
